Adaptive Tensegrity Locomotion on Rough Terrain via Reinforcement Learning

The dynamical properties of tensegrity robots give them appealing ruggedness and adaptability, but present major challenges with respect to locomotion control. Due to high-dimensionality and complex contact responses, data-driven approaches are apt for producing viable feedback policies. Guided Policy Search (GPS), a sample-efficient and model-free hybrid framework for optimization and reinforcement learning, has recently been used to produce periodic locomotion for a spherical 6-bar tensegrity robot on flat or slightly varied surfaces. This work provides an extension to non-periodic locomotion and achieves rough terrain traversal, which requires more broadly varied, adaptive, and non-periodic rover behavior. The contribution alters the control optimization step of GPS, which locally fits and exploits surrogate models of the dynamics, and employs the existing supervised learning step. The proposed solution incorporates new processes to ensure effective local modeling despite the disorganized nature of sample data in rough terrain locomotion. Demonstrations in simulation reveal that the resulting controller sustains the highly adaptive behavior necessary to reliably traverse rough terrain.

==> makefile <==
DOCUMENT  := tensegrity_terrain

.PHONY: latex

TEMPLDIR   := ~/repositories/templates/latex

FORMATDIR  := ../format:$(TEMPLDIR)/packages:$(TEMPLDIR)/ieee_format:$(TEMPLDIR)/acm_format:$(TEMPLDIR)/kostas_style:$(TEMPLDIR)/other_format:../$(TEMPLDIR)/ieee_format:../$(TEMPLDIR)/acm_format:../$(TEMPLDIR)/kostas_style:../$(TEMPLDIR)/other_format
FIGUREDIR  := ../figures
BIBDIR     := ../bib
BINDIR     := ./bin

DVI_OPTIONS := -Ppdf -G0 -tletter
PS2PDF_OPTIONS := -dCompatibilityLevel=1.3 -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter

export TEXINPUTS=.:$(FORMATDIR):$(FIGUREDIR)::
export BIBINPUTS=.:$(BIBDIR)::
export BSTINPUTS=.:$(FORMATDIR):$(BIBDIR)::

export TEXMFOUTPUT=$(PWD)

latex:
	rubber -v --pdf --warn=all --into $(BINDIR) $(DOCUMENT).tex

clean:
	rubber --pdf --into $(BINDIR) --clean $(DOCUMENT).tex
	\rm -rf bin/*out


==> related_work.tex <==
%%%% OUTLINE
%
% General control/planning for high-dim dynamic systems
%   * 
%   * 
%   * 
%   
% Tensegrity applications of 
%   * System complexity
%   * Control



\subsection{Tensegrity Control}

Couple paras on model-based

Couple paras on CPGs, evolutionary algorithms, other older stuff

%%% Stuff that's new since I last did much literature search on tensegrity

Small-scale 6 bar tensegrity - ascend slope with 2-cable actuation scheme. 26 deg (alternating two-cable), 24 deg (simultaneous two-cable).  Smooth slope, experienced slipping at around 23 to 29 deg. Also saw this in NTRT simulation.
~\cite{chen_inclined_2017}.


Uses MDGPS, analyze different small observation spaces.  TT4 is 6-bar, 24-motor.  Periodic gait.
Claims:
1) success despite low-dim obs space (zhang obs space was p low though).
2) evaluations, demonstration with 3d obs space
3) "motivate research into previously unexplored deep rl algorithms" wtf? "and demonstrate... on rough terrains" (terrains not at all rough).  
Paper is actually quite sloppy.  
Sample complexity sounds fairly low, and yet, 4 hour runtime...
Newly applies Path Integral GPS.
"Rough terrain" looks like maybe 3-5\% of a bar length.
Refers to terrain as causing the dynamics to become discontinuous...
~\cite{agogino18}.




\subsection{Guided Policy Search}

Other systems it has been applied on -- mostly rather low dimension

Previous fixed-axis application



